Exploratory Not Explanatory: Counterfactual Analysis of Saliency Maps for Deep Reinforcement Learning

Saliency maps are frequently used to support explanations of the behavior of deep reinforcement learning (RL) agents. However, a review of how saliency maps are used in practice indicates that the derived explanations are often unfalsifiable and can be highly subjective. We introduce an empirical approach grounded in counterfactual reasoning to test the hypotheses generated from saliency maps and assess the degree to which they correspond to the semantics of RL environments. We use Atari games, a common benchmark for deep RL, to evaluate three types of saliency maps. Our results show the extent to which existing claims about Atari games can be evaluated and suggest that saliency maps are best viewed as an exploratory tool rather than an explanatory tool.

==> ICLR%202020%20--%20Evaluating%20Saliency%20Maps%20for%20Deep%20RL%20Using%20Counterfactual%20Reasoning(1)/buffet.tex <==
\begin{abstract}
  Visualization tools are often employed to evaluate, explain, and debug deep networks. Saliency maps are a popular method that produce heatmap-like output highlighting the importance of different regions of the input. Recent work in deep reinforcement learning (RL) has emphasized deriving interpretable saliency maps with the belief that they will facilitate explanations over temporally extended sequences. However, our survey of their use in the community indicates that the explanations derived from saliency maps are often unfalsifiable and can be highly subjective. %, and the literature offers limited evidence that deep RL agents are using representations of human-understandable concepts. 
  %Given the established connection between explanation and causal reasoning in the causal inference literature, it is important to determine whether saliency maps reflect causal relationships between an agent's behavior and its environment. 
  We propose an empirical approach to verify the hypotheses generated from saliency maps for deep RL and provide a methodology to evaluate the causal relationship between semantic concepts and saliency maps. We evaluate two general categories of saliency maps, gradient-based and perturbation-based, using Atari games, a common benchmark for deep RL. 
  %To generate interventional data, we use Toybox, a fully parameterized implementation of three Atari games. This provides a novel framework for evaluating saliency maps under intervention. 
  Our results show the extent to which existing claims about Atari games can be evaluated and provide evidence for whether saliency maps are suitable for causal interpretation.
\end{abstract}

% Introduction

% scene setting
%The promising performance of deep reinforcement learning (RL) agents \citep{mnih2015human} has laid the foundations for modern goal-oriented algorithms.
% State-of-the-art deep RL agents have demonstrated promising performance in various domains including video games \citep{mnih2015human,vinyals2017starcraft, lample2017playing,silver2017mastering,Brown418}, robotics \citep{gu2017deep, zhu2017target} and autonomous driving \citep{sallab2017deep, shalev2016safe}. Yet, these methods are often criticized for their lack of interpretability and explainability.

% \kaleigh{TODO}: discussion of interpretability and explainability of deep nets

%They were first introduced in the deep neural network (DNN) literature by \cite{simonyan2013deep} and their use as explanations of network decisions has led to significant efforts in producing human-interpretable saliency maps. 
%In spite of their success with DNNs, the complexity rises in deep RL environments where decisions in aggregate correspond to agent behavior over temporally extended sequences of frames. %Some researchers have attempted to use saliency maps to provide evidence for explanations of agent behavior in deep RL \citep{greydanus2017visualizing, sundar2018transparency, iyer2018transparency}.

% This is different from image classification tasks where the network is typically provided a single image as input. Deep RL agents are structured differently to explore an environment, such as an Atari game, during training and expected to learn a policy. Thus, explanations in this context require more complex reasoning as they are derived from a temporal sequence of actions

%To generate interventional data, we use Toybox, a fully parameterized implementation of three Atari games \citep{foley2018toybox}. This provides a novel framework for evaluating saliency maps under intervention for RL environments. 
% We conducted a survey to better understand the ways in which saliency maps have been used as evidence in explanations of deep RL agents and found that saliency maps have been used to support explanations relating to semantic concepts of RL environments.
%Our survey suggests that saliency maps are often used for two main tasks: (1) assessing the RL agent's learned representations of semantic concepts, and (2) identifying the semantic features used for policy construction.

%Since saliency maps in deep RL are derived from a stack of temporally contiguous frames, 
% Since understanding environment semantics is particularly important for the success of deep RL agents, ascribing meaning to pixel-level interventions requires more scrutiny; 
%Our survey finds that saliency maps have been used to support explanations relating to semantic concepts of RL environments. However, the results communicated with saliency maps may not apply to human-understandable concepts. 
% The explanations that researchers frequently derive from saliency maps may not correspond to semantic concepts and features of RL environments. If saliency maps do not reflect the interventional relationships that are assumed by some researchers, incorrect, extrapolated conclusions may be drawn from the resulting maps.

% motivation
% \textbf{Survey of Usage of Saliency Maps.} We conducted a survey of how the deep RL community uses saliency maps and found that the explanations derived from saliency maps are often unfalsifiable, and can be highly subjective given the volume of conceptual information in image-based RL environments. We hypothesize that saliency maps are not self-sufficient to interpret RL agents and must be used with other evaluation methods.

%\textbf{Causal Explanations from Saliency Maps.}  %If saliency maps are used as tools of explanation, they should reflect causal relationships between the RL environment and the agent's behavior. 

% \textbf{Assessing Learned Representations from Saliency.} The explanations derived from saliency maps typically involve \textit{semantic}, human-understandable concepts. That is, salient pixels are typically mapped directly to semantic concepts in a game. However, the literature offers limited evidence that saliency maps are causally dependent on representations of human-understandable concepts. Recent work provides evidence for deep networks and humans having different visual inspectors \citep{}.

% \textbf{Assessing Inferred Policy Construction from Saliency.}


%approach
% \textbf{Example.} Consider the causal graphical model in Figure \ref{simple_gm} for an Atari game. The RL framework consists of the environment (in blue) and system (in yellow). In the environment, the \textit{pixel input} is generated from the underlying \textit{game state}. Then, pixel input and the \textit{learned network} are used to predict \textit{logits}, the raw probabilities over the output space. \textit{Saliency maps} are generated from the output of these logits and logits in aggregate also influence the agent's \textit{behavior}, such as "aiming". The game state affects \textit{semantic concepts} of the game. Together, saliency maps, behavior and semantic concepts are typically employed to generate explanations or \textit{claims} about agent behavior over temporally extended sequences.

% As described above, researchers assume saliency maps have a causal relationship with an agent's behavior and its environment. However, to the best of our knowledge, there is little evidence supporting this assumption. To test this hypothesis, we intervene on the common cause of behavior and saliency maps by following the causal chain back to game state. We intervene on game state, which is typically latent, using Toybox such that the underlying behavior holds true for a temporally extended sequence of frames. If the saliency maps do reflect this change, we can reject our hypothesis. Similarly, we can also verify how well semantic concepts correlate with salient pixels.

% Our experiments show some interesting results. TODO: add summary of results.

% outline, can be optional depending on venue/audience 
% Our paper proceeds as follows: ...

%It is noteworthy that all three of these components are connected only via common causes (i.e. pixel input and model). Hence, a connection between the components does not imply that a causal relationship exists. This alludes to the importance of assessing the degree to which saliency maps meet the assumptions outlined in section \ref{sec-inadeq} to determine whether saliency maps are good explanatory tools.


\subsection{Saliency Maps}
%Background on SMs
\subsubsection{Saliency Maps in Computer Vision}
% Saliency maps in the supervised DNN literature can be categorized into two categories.

\textbf{Gradient-Based Saliency.} Saliency maps were introduced by \citet{simonyan2013deep} to determine what pixels of an image are the most relevant to the network's decision. This involves calculating the gradient of the output with respect to the input.
%Using un-normalized scores of all the classes $S_c$ from a forward pass of the DNN, the authors back-propagate on the gradients with respect to the input $I$, $w_{ij}^c = \frac{\partial S_c}{\partial I} \arrowvert_{I_0}$, to get the pixel saliency at location $(i,j)$. A class saliency map can be generated by normalizing over the image for all pixel locations: $M_c(i,j) = \frac{w_{ij}}{\sum_{ij} w_{ij}}$. 
Following \cite{simonyan2013deep}, a multitude of gradient-based methods have been developed for DNNs with the intention of getting more realistic and understandable saliency maps \citep{simonyan2013deep, springenberg2014striving, shrikumar2017learning, smilkov2017smoothgrad, selvaraju2017grad, zhang2018top}. %For instance, Guided Backpropagation \citep{springenberg2014striving}, DeepLIFT \citep{shrikumar2017learning}, SmoothGrad \citep{smilkov2017smoothgrad}, Grad-CAM \citep{selvaraju2017grad} and most recently, Excitation Backpropagation \citep{zhang2018top} have been introduced.

\textbf{Perturbation-Based Saliency.} An alternative to gradient-based saliency map methods is perturbation-based methods. They were developed to measure how a change in conceptual parts of the input alters the network's output \citep{zeiler2014visualizing}. However, a common issue with this approach is it is difficult to perturb an area without introducing new information. Various other methods have been introduced to perturb pixels such that minimal new information is introduced \citep{ribeiro2016should, dabkowski2017real, fong2017interpretable}.  %This was first introduced by \cite{zeiler2014visualizing}, where the authors introduced masking portions of an image with gray squares to identify whether the network is using objects or the surrounding context. However, a common issue is this introduces new information, which hinders with the reasoning behind perturbing. Another variant of this is perturbation-based pixel saliency \citep{ribeiro2016should}. Advanced masking methods have been introduced by \cite{dabkowski2017real}, and \cite{fong2017interpretable}. Both of these use masked interpolation through an image to introduce minimal new information with the perturbation.

Background

% \section{Background}
% %Background on deep RL
% \subsection{Deep Reinforcement Learning}
% Reinforcement learning is a subfield of machine learning interested in training an agent to act in an environment through interaction. Certain states in the environment give the agent positive or negative reward. The agent learns a \emph{policy}, a mapping between states $S$ and actions $A$ according to reward signals $r \in R$. The goal is to learn a policy $\pi$ that maximizes the discounted sum of rewards received while acting in the environment \citep{sutton1998reinforcement}. 

% Deep reinforcement learning uses deep neural networks to represent policies. These models enable interactions using high-dimensional state inputs (e.g., images). % the hope is that it learns its own visual features for policy representation


%Use of SMs in the RL community.
% \subsection{Saliency Maps in Deep RL} 
% There is a growing use of saliency maps in deep RL. We consider four general categories of saliency maps in deep RL.
%There are a few saliency map methods available in this paradigm.

% \textbf{Jacobian Saliency.} Jacobian saliency maps, an application of regular gradient-based saliency maps, have been used to visualize the outputs of DQNs and generate explanations \citep{wang2015dueling, zahavy2016graying, bogdanovic2015deep}. However, as \cite{sundar2018transparency} point out, gradient-based methods in DNNs approximate linear decision boundaries and this does not produce interpretable saliency maps in deep RL because the mapping from states to actions is highly diverse unlike input image to class label mapping in classification tasks.
% %Sundar et al: "Pixel saliency makes linear approximations of the decision boundary and hence com-putes only local gradients.   GradCAM combines class specific gradient informationflowing into the last convolutional layer of the CNN. While this is useful for super-vised learning, this may not yield good saliency maps for reinforcement learning. Thisis because the reinforcement learning networks are not trained for an input image toclass label mapping and there is a high diversity in the input states for which the net-work chooses an action label “UP” for instance. "
% % \citet{sundar2018transparency} showed multiple gradient-based saliency maps on Atari testbeds and their substantially differing resulting interpretations. 
% Thus, merely porting saliency map methods from supervised contexts to deep RL does not fulfill the purposes that explanations in RL require. In this work, we use Jacobian saliency maps as the baseline. 

% \textbf{Perturbation Saliency.} Recognizing the lack of interpretability in Jacobian saliency methods, \citet{greydanus2017visualizing} developed a perturbation-based method to generate saliency videos of deep RL agents. They perturb the original input image using a Gaussian blur of the image generated by the Hadamard product and measure changes in policy from removing information from a region. TODO: add details how this is a less fat-handy perturbation and why that is important in the case of RL.

% \textbf{Object Saliency.} Noting the importance of objects in RL testbeds, \citet{iyer2018transparency} developed an object-sensitive saliency visualization method. They use template matching, a common computer vision technique, to detect (template) objects within an input image and store these in \textit{object channels} in the input image alongside the RBG channels. To generate object sensitive saliency maps, they mask each object with the background image and compute the difference in Q-values of the unmasked and masked states. The difference in Q-values represent the influence of the object on the Q-value.

% \textbf{Attention Saliency.} Most recently, attention-based methods have been proposed to generate interpretable saliency maps \citep{mott2019towards, nikulin2019free}.

% Saliency map methods typically use backpropogation of activations to identify parts of the images most important to making the agent’s decision. Briefly describe:
% \begin{itemize}
%     \item Jacobian methods
%     \item perturbation methods
%     \item the type surviving the Kim et al 2018 analysis (Guided Backprop?) \citep{adebayo2018sanity}
% \end{itemize}

% Saliency maps have been used to support explanations of agent behavior in RL applications \citep{}. Discussion:
% \begin{itemize}
%     \item why the temporal component makes reasoning harder in general; especially so in the case of porting SM methods from supervised contexts to RL
%     \item what methods are used/available in this paradigm 
%     \item use in the RL community for explanation 
% \end{itemize}

\subsection{Evaluation of Semantic Concepts in Saliency Maps}
To identify when there is a relationship between semantic concepts and saliency, we empirically evaluate the counterfactual importance of each semantic concept. We first identify semantic concepts using the extended graphical models (see appendix). We then design and run 50 samples of each intervention for each semantic concept. The interventions are run with varying intensities for 150 timesteps. See Table \ref{interventions} for a description of the interventions.

\begin{table}
\centering
\begin{tabular}{ |c|c|c| } 
 \hline
     & \textbf{Concepts} & \textbf{Intervention} \\ 
 \hline
 \textbf{Breakout} & Ball & \textbf{(1)} move ball position between [5,15] pixels; \textbf{(2)} increase ball speed by [1,3]. \\ 
  & Paddle & \textbf{(1)} move paddle position between [5,15] pixels to left or right. \\ 
  & Bricks & \textbf{(1)} invert bricks; \textbf{(2)} remove 5 random bricks; \textbf{(3)} remove a random row. \\ 
 \hline
 \textbf{Amidar} & Player & 4  \\ 
  & Enemies & 36 \\
  & Tiles & 36 \\
 \hline
\end{tabular}
\caption{Interventions for identifying CFi for each semantic concept.}
\label{interventions}
\end{table}

The results for the relationship between CFi and saliency in Breakout are shown for each intervention in Figure \ref{breakout_cfi_corr}. TODO: explain results. 

Similar experiments are done for Amidar (see appendix X). We find...TODO: explain results for Amidar. 

It could be that the relationship between CFi and saliency only holds at certain time periods (i.e. when ball is near the paddle in Breakout). To identify this, we assess if there is a pattern between CFi and salient over time. The results can be found in Figure \ref{}. We expect to see that CFi and saliency peak at the same time for the causal relationship to hold. TODO: explain results.

\begin{figure}
    \hspace*{-1cm}        
    \centering
    \includegraphics[width=\linewidth]{figures/breakout_CFi_saliency_corr_50s.png}
    \caption{Counterfactual importance vs saliency for (a) perturbation saliency; (b) object saliency; (c) Jacobian saliency.}
    \label{breakout_cfi_corr}
\end{figure}


%Reinforcement learning is complicated, and deep networks are complicated. There is a real need for explanation in these systems. Deep models in reinforcement learning are used for selecting actions over temporally extended periods. The temporal and interactive nature of RL systems present a different set of opportunities and challenges in explanations of behavior. Given the development and use of saliency maps to support explanations of agent behavior in deep RL applications, the use of saliency maps as tools of explanation in RL deserves its own evaluation.

\begin{figure}
\centering
	\begin{minipage}{.3\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/breakout_control.png}
		%\caption{original}
		\label{fig:breakout_control}
		\end{minipage}
%
	\begin{minipage}{.3\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/breakout_reflect.png}
		%\caption{reflected}
		\label{fig:breakout_reflect}
	\end{minipage}
	
	\begin{minipage}{.3\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/breakout_reflect_bp.png}
		%\caption{reflected}
		\label{fig:breakout_reflect_bp}
	\end{minipage}
\caption{(a) A perturbation saliency map from a frame in Breakout, and (b) a saliency map from the same model on the same frame with the brick patterned reflected across the vertical axis. \akanksha{The red regions indicate areas of the image that represent rewards, and blue regions indicate areas of the image that represent actions}. The pattern and intensity of saliency around the channel is not symmetric. In Section \ref{sec:case-study-1}, we examine whether reflecting the ball and paddle positions with the brick configuration increases the saliency of the reflected channel. }
\label{fig:breakout_example}
\end{figure}

\section{Generating Claims}
Note the inverse of the proposed approach is \textit{sufficiently causal}: TODO: give definition. If the agent has learned representation $R$, the pixels corresponding to the learned representation will always be salient. However, another learned representation may result in saliency on the same set of pixels. Researchers are instead interested in inferring what the agent has learned using saliency. This is also known as inferring \textit{causes of effects}. 

\textbf{Assessing Policy Construction.}
% The survey reveals that researchers associate intent behind policy construction and associate behavioral features. 
The policy a deep RL agent learns during training is guided by reward signals in the environment. These reward signals map to how the semantic features in the game evolve. By definition, these representations are causal for the network's output and are consequently reflected in saliency maps. However, given the many-to-many mapping between semantic concepts...
% The policy a deep RL agent learns during training contains what humans see as behavioral features. These representations are causal for the network's output and are consequently reflected in saliency maps. However, there are various other associational representations that can be speculated from a saliency map despite them not existing in the learned policy. \cite{???} provided evidence that humans are more susceptible to identifying spurious correlations. This suggests that any human reasoning requires complex interpretation to assess learned representations from saliency maps.

\textbf{Assessing Learned Representations.}
Prior studies have provided evidence that humans rely on references to semantic, human-understandable concepts. \cite{tenenbaum2003learning} demonstrate that humans organize objects based on their causal properties and inherently form abstract categories. \cite{dubey2018investigating} further show that humans use semantic concepts to develop a strategy to play games. Similarly, the survey reveals that humans look at saliency maps and interpret a strategy by associating salient pixels with concepts they know of. However, there is little evidence that saliency maps are capable of representing complex semantic-level representation.

\section{Assumptions}
To interpret saliency maps as explanatory tools for deep RL, researchers typically make the following assumptions. 
First, saliency maps indicate constraints on the space of possible policies. For instance, the example above uses saliency to assess that the agent has learned to ``target bricks with higher reward.''
Second, salient regions capture representations of semantic concepts learned by the network. 
For instance, the salient region above the tunnel being created in Figure \ref{fig:breakout_example}a can easily be interpreted to indicate the importance of tunnels to the agent.

\section{CF Importance}
%CF importance; what matters and what doesn’t for agent
% \textbf{Evaluating Existence of Semantic Concepts in Saliency Maps.} To evaluate the relationship between semantic concepts and saliency maps, we propose identifying the \textit{counterfactual importance} of each semantic concept. We define counterfactual importance (CFi) as $CFi (A_f, A_c) = \sqrt{\sum_{i=0}^{n} (A_f(i) - A_c(i))^2}$ where $A_f$ and $A_c$ are the probability distributions over the set of actions for a factual and counterfactual state respectively, and $n$ is the number of actions. Counterfactual importance intuitively reflects what is significant to the agent versus what is not at a given state. We expect that if a semantic concept is highly salient, intervening on it should result in a different distribution over actions (i.e. CFi). If the intervention causes a higher CFi for a highly salient ojbect, this implies that there is a causal relationship the semantic concept and saliency. We can similarly calculate the counterfactual importance using the value output.

% Figures \ref{amidar_score_ex_pert} and \ref{amidar_score_ex_jac} show the result of intervening on displayed score on reward and saliency intensity for the first 1000 timesteps of an episode. The mean is calculated over 50 samples. If an agent died before 1000 timesteps, the last reward was extended for the remainder of the timesteps and saliency was treated to be non-existent (ie. 0).  %show a contradicting example of saliency maps not being causally affected by agent behavior. That is 

% Using rewards as a proxy for agent behavior, we can conclude that different interventions on score produce contrasting agent behavior. This is evident from rewards differing over time for all the interventions due to early agent death.
% However, salience intensity patterns of all interventions follow very closely to the original trajectory. Since various interventions on displayed score cause degraded performance (Figure \ref{amidar_score_ex_obj}b) despite resulting in similar saliency maps (Figure \ref{amidar_score_ex_obj}c), we can conclude that we cannot assess the agent's behavior using just saliency intensity.

==> ICLR%202020%20--%20Evaluating%20Saliency%20Maps%20for%20Deep%20RL%20Using%20Counterfactual%20Reasoning(1)/claims.tex <==
\definecolor{lightgray}{gray}{0.85}
\renewcommand{\arraystretch}{1.25}
\begin{longtable}{p{0.5\linewidth}*{2}{p{0.1\linewidth}}*{2}{c}}
\hline
  \rowcolor{lightgray} \multicolumn{1}{c}{Claim}  & \multicolumn{1}{c}{Game} & Saliency Type & Reason & Exp \\
  \toprule
  \multicolumn{5}{c}{\citet{greydanus2017visualizing}}\\
  %\hline
  ``The agent is positioning its own paddle, which allows it to return the ball at a specific angle.''  & Pong & Perturbation & Y & N \\ 
  ``Interestingly, from the saliency we see that the agent attends to very little besides its own paddle: not even the ball.'' &  Pong & Perturbation & N & N \\ 

  ``After the agent has executed the kill shot, we see that saliency centers entirely around the ball. This makes sense since at this point neither paddle can alter the outcome and their positions are irrelevant.'' & Pong & Perturbation & Y & N \\ 
  ``It appears that the deep RL agent is exploiting the deterministic nature of the Pong environment. It has learned that it can obtain a reward with high certainty upon executing a precise series of actions. This insight...gives evidence that the agent is not robust and has overfit to the particular opponent.''  & Pong & Perturbation & Y & N \\ 
``[The agent] had learned a sophisticated aiming strategy during which first the actor and then the critic would `track' a target. Aiming begins when the actor highlights a particular alien in blue...Aiming ends with the agent shooting at the new target.''  & Space\-Invaders & Perturbation & Y & N \\ 
 ``The critic highlights the target in anticipation of an upcoming reward.''   & Space\-Invaders & Perturbation & Y & N \\ 
 ``Notice that both actor and critic tend to monitor the area above the ship. This may be useful for determining whether the ship is protected from enemy fire or has a clear shot at enemies.''   & Space\-Invaders & Perturbation & Y & N  \\ 
 ``We found that the agent enters and exits a `tunneling mode' over the course of a single frame. Once the tunneling location becomes salient, it remains so until the tunnel is finished.''  & Break\-out & Perturbation & N & N \\ 
\toprule
\multicolumn{5}{c}{\citet{zahavy2016graying}}\\
%\hline
``A diver is noticed in the saliency map but misunderstood as an enemy and being shot at.''  & Sea\-quest & Jacobian & Y & N \\ 
 ``Once the agent finished the first screen it is presented with another one, distinguished only by the score that was accumulated in the first screen. Therefore, an agent might encounter problems with generalizing to the new screen if it over-fits the score pixels. Figure 15 shows the saliency maps of different games supporting our claim that DQN is basing its estimates using these pixels. We suggest to further investigate this, for example, we suggest to train an agent that does not receive those pixels as input.''  & Breakout & Jacobian & N & N \\ 
 \toprule
 \multicolumn{5}{c}{\citet{bogdanovic2015deep}} \\
 ``The line of cars in the upper right are far away and the agent correctly ignores them in favour of focusing on the much more dangerous cars in the lower left.'' & Freeway & Jacobian & Y & N \\ 
  \toprule
  \multicolumn{5}{c}{\citet{yang2018learn}}\\
 ``Firstly, the agent ignores irrelevant features from mountains, sky, the mileage board and empty grounds, and relies on information from the race track to make decisions.  Specifically, the agent keeps separate two categories of objects on the race track, i.e., cars and the player.''  & Enduro & Binary Jacobian & Y & N \\ 
 ``On the one hand, the agent locates the player and a local area around it for avoiding immediate collisions with cars.  On the other hand, the agent locates the next potential collision targets at different locations, particularly the remote ones.''  & Enduro & Binary Jacobian & Y & N \\ 
 ``Near the completion of the current goal, the agent “celebrates” in advance. As shown from Fig. 4(d) to Fig. 4(f), the left gaze loses its focus on cars and diverts to the mileage board starting when only 13 cars remain before completion. The previous “car tracker” now picks up on the “important” information that it is close to victory, and fixates on the countdown.'' & Enduro & Binary Jacobian & Y & N \\ 
``Upon reaching the target, the agent does not receive reward signals until the next day starts. During this period the agent learns to output no-op actions, corresponding to not playing the game.'' & Enduro & Binary Jacobian & Y & N \\ 
 ``When slacking happens, the agent considers the flag signs as important and the road not.  The complete reverse in focus as compared to the normal case explains this shift in policy.  The flags outweigh the road in importance, since they are signs of absolute zero return." & Enduro & Binary Jacobian & Y & N \\ 
  ``(Prepping) As it turns out, the agent recognizes that the time is dawn (right before morning when race starts) from the unique colours of the light gray sky and orange mountains, therefore the agent gets ready early for a head start in the new race.'' & Enduro & Binary Jacobian & Y & N \\ 
  ``When smog partially blocks the forward view, the left gaze loses its focus on cars. It strays off the road into some empty area.'' &  Enduro & Binary Jacobian & Y & N \\ 
  ``In Fig. 5(a), the left gaze detects the two ghosts on the upper-right corner of the map. Therefore, ms pacman, as located by the right gaze, stays in the mid-left section to safely collect dense rewards. '' & Pacman & Binary Jacobian & Y & N \\ 
  ``In Fig. 5(b), the left gaze locks in on all three vulnerable ghosts in the mid-right section, as ms pacman chases after them.'' & Pacman & Binary Jacobian & Y & N \\ 
  ``In Fig. 5(c), the left gaze detects a newly-appeared cherry at the lower-left warp tunnel entrance. Ms pacman immediately enters the closest opposite tunnel entrance in the shortest path to the cherry.'' & Pacman & Binary Jacobian & Y & N \\ 
 ``In Fig. 5(d), the right gaze locates ms pacman entering the upper-right tunnel. In this case, the left gaze no longer detects a moving object, but predicts the upper-left tunnel as the exiting point.'' & Pacman & Binary Jacobian & Y & N \\ 
 ``As shown in Fig. 5(g), the left gaze locates the last pellet when ms pacman is in the mid-section of the maze. Therefore ms pacman moves towards the pellet.'' & Pacman & Binary Jacobian & Y & N \\ 
 ``In Fig. 5(h), a red ghost appears in the left gaze close to the pellet, causing ms pacman to deviate to the right.'' & Pacman & Binary Jacobian & Y & N \\ 
 ``After changing course, the ghosts approach ms pacman from all directions as shown in Fig. 5(i). Even though the agent detects all the ghosts (they appear in the gazes), ms pacman has no route to escape.'' & Pacman & Binary Jacobian & Y & N \\ 
 ``The left gaze often focuses on white ice blocks that are the destinations of jumping.'' & Frostbite & Binary Jacobian & N & N \\ 
 ``Fig. 6(b) shows the sub-task of the player entering the igloo, after jumping over white ice blocks for building it. The player must avoid the bear when running for the igloo.'' & Frostbite & Binary Jacobian & Y & N \\ 
 ``As it shows, the igloo is two jumps away from completion, and the left gaze focuses on the igloo in advance for preparing to enter.'' & Frostbite & Binary Jacobian & Y & N \\ 
 \toprule
 \multicolumn{5}{c}{\citet{annasamy2019towards}}\\
 ``For example, in MsPacman, since visualizations suggest that the agent may be memorizing pacman’s positions (also maybe ghosts and other objects), we simply add an extra pellet adjacent to a trajectory seen during training (Figure 7a). The agent does not clear the additional pellet and simply continues to execute actions performed during training (Figure 7b).'' & Pacman & Object & Y & Y \\ 
 ``Similarly, in case of SpaceInvaders, the agent has a strong bias towards shooting from the leftmost-end (seen in Figure 4). This helps in clearing the triangle like shape and moving to the next level (Figure 7d). However, when triangular positions of spaceships are inverted, the agent repeats the same strategy of trying to shoot from left and fails to clear ships (Figure 7c).'' & Space\-Invaders & Object & Y & Y \\ 
 \newpage
 \toprule
 \multicolumn{5}{c}{\citet{goel2018unsupervised}}\\
 ``In our Breakout results, the network learns to split the paddle into a left and right side, and does not move the middle portion.'' & Breakout & Object & Y & N \\ 
``On Beam Rider, our network achieves low loss after learning to segment the game’s light beams, however these beams are purely visual effects and are unimportant for action selection.'' & Beam Rider & Object & Y & N \\
 ``Consequently, the game enemies, which are much smaller in size, are ignored by the network, and the resulting learned representation is not that useful for a reinforcement learning agent.'' & Beam Rider & Object & N & N \\ 
 \toprule
 \multicolumn{5}{c}{\citet{van2018advantage}}
\\
``There is a very notable difference between the policy saliency between the two models, where the former one only pays limited attention to the road and almost no attention to the engine indicator, the opposite from fA3C-LSTM. Explicitly,it means masking any regions from the input does not cause much perturbation to the policy when trained with continuous space as targets, likely because the real consequence from a small change in action, e.g.  no braking (a3= 0) versus braking (a3= 0.3), can be very substantial but numerically too subtle for the network to capture during optimization on the continuous spectrum.'' & CarRacing & Perturbation & Y & N \\ 
\toprule
 \multicolumn{5}{c}{\citet{rupprecht2018visualizing}} \\
 ``Analyzing the visualizations on Seaquest, we make an interesting observation. When maximizing the Q-value for the actions, in many samples we see a low or very low oxygen meter. In these cases the submarine would need to ascend to the surface to avoid suffocation. Although the up action is the only sensible choice in this case, we also obtain visualized low oxygen states for all other actions. This implies that the agent has not understood the importance of resurfacing when the oxygen is low. We then run several roll outs of the agent and see that the major cause of death is indeed suffocation and not collision with enemies.'' & SeaQuest & Perturbation & Y & Y \\
 \toprule
 \multicolumn{5}{c}{\citet{mott2019towards}}\\
 ``The most dominant pattern we observe is that the model learns to attend to task-relevant things in the scene. In most ATARI games that usually means that the player is one of the foci of attention, as well as enemies, power-ups and the score itself (which is an important factor in the calculating the value function).'' & SeaQuest & Attention & N & N \\ 
 ``Figure 4 shows a examples of this in Ms Pacman and Alien — in the both games the model scans through possible paths, making sure there are no enemies or ghosts ahead. We observe that when it does see a ghost, another path is produced or executed in order to avoid it.'' & Pacman & Attention & Y & N \\ 
 ``In many games we observe that the agent learns to place “trip-wires” at strategic points in space such that if a game object crosses them a specific action is taken. For example, in Space Invaders two such trip wires are following the player ship on both sides such that if a bullet crosses one of them the agent immediately evades them by moving towards the opposite direction.'' & Space Invaders & Attention & Y & N \\ 
 ``Another example is Breakout where we can see it working in two stages. First the attention is spread out around the general area of the ball, then focuses into a localized line. Once the ball crosses that line the agent moves towards the ball.'' & Breakout & Attention & Y & N \\ 
  ``As can be seen, the system uses the two modes to make its decisions, some of the heads are content specific looking for opponent cars. Some are mixed, scanning the horizon for incoming cars and when found, tracking them, and some are location based queries, scanning the area right in front of the player for anything the crosses its path (a “trip-wire” which moves with the player).'' & Enduro & Attention & Y & N \\ 
 ``Comparing the attention agent to the baseline agent, we see that the attention agent is sensitive to more focused areas along the possible future trajectory. The baseline agent is more focused on the area immediately in front of the player (for the policy saliency) and on the score, while the attention agent focuses more specifically on the path the agent will follow (for the policy) and on possible future longer term paths (for the value).'' & Pacman & Perturbation & Y & N \\ 
 \toprule
 \multicolumn{5}{c}{\citet{nikulin2019free}}\\
 ``Figs. 4(a)-(b) show Dense FLS digging a tunnel through blocks in Breakout. The model focuses its attention on the end of the tunnel as soon as it is complete, suggesting that it sees shooting the ball through the tunnel as a good strategy.'' & Breakout & Attention & Y & N \\ 
  ``Figs. 4(c)-(d) depict the same concept of tunneling per-formed  by  theSparse  FLSmodel.   Note  how  it  focuses attention on the upper part of the screen after destroying multiple bricks from the top.  This attention does not go away after the ball moves elsewhere (not shown in the images).We speculate that this is how the agent models tunneling:rather than having a high-level concept of digging a tunnel,it simply strikes wherever it has managed to strike already.'' & Breakout & Attention & Y & N \\ 
  ``Figs. 4(e)-(f) illustrate how the Dense FLS model playing Seaquest has learned to attend to in-game objects and, importantly, the oxygen bar at the bottom of the screen. As the oxygen bar is nearing depletion, attention focuses around it,and the submarine reacts by rising to refill its air supply.'' & Seaquest & Attention & Y & N \\ 
  ``Figs. 4(g)-(h) are two consecutive frames where an agent detects a target appearing from the left side of the screen.The bottom part of the screenshots shows how attention in the bottom left corner lights up as soon as a tiny part of the target, only a few pixels wide, appears from the left edge of the screen.  In the next frame,  the agent will turn left and shoot the target (not shown here). However, the agent completely ignores targets in the top part of the screen, and its attention does not move as they move (also not shown).'' & Breakout & Attention & Y & N \\ 
 \toprule
 \multicolumn{5}{c}{\citet{wang2015dueling}}\\
  ``The value stream learns to pay attention to the road. The advantage stream learns to pay attention only when there are cars immediately in front, so as to avoid collisions.''  & Enduro & Jacobian & Y & N 
\end{longtable}


==> ICLR%202020%20--%20Evaluating%20Saliency%20Maps%20for%20Deep%20RL%20Using%20Counterfactual%20Reasoning(1)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> buffet.tex <==
\begin{abstract}
  Visualization tools are often employed to evaluate, explain, and debug deep networks. Saliency maps are a popular method that produce heatmap-like output highlighting the importance of different regions of the input. Recent work in deep reinforcement learning (RL) has emphasized deriving interpretable saliency maps with the belief that they will facilitate explanations over temporally extended sequences. However, our survey of their use in the community indicates that the explanations derived from saliency maps are often unfalsifiable and can be highly subjective. %, and the literature offers limited evidence that deep RL agents are using representations of human-understandable concepts. 
  %Given the established connection between explanation and causal reasoning in the causal inference literature, it is important to determine whether saliency maps reflect causal relationships between an agent's behavior and its environment. 
  We propose an empirical approach to verify the hypotheses generated from saliency maps for deep RL and provide a methodology to evaluate the causal relationship between semantic concepts and saliency maps. We evaluate two general categories of saliency maps, gradient-based and perturbation-based, using Atari games, a common benchmark for deep RL. 
  %To generate interventional data, we use Toybox, a fully parameterized implementation of three Atari games. This provides a novel framework for evaluating saliency maps under intervention. 
  Our results show the extent to which existing claims about Atari games can be evaluated and provide evidence for whether saliency maps are suitable for causal interpretation.
\end{abstract}

% Introduction

% scene setting
%The promising performance of deep reinforcement learning (RL) agents \citep{mnih2015human} has laid the foundations for modern goal-oriented algorithms.
% State-of-the-art deep RL agents have demonstrated promising performance in various domains including video games \citep{mnih2015human,vinyals2017starcraft, lample2017playing,silver2017mastering,Brown418}, robotics \citep{gu2017deep, zhu2017target} and autonomous driving \citep{sallab2017deep, shalev2016safe}. Yet, these methods are often criticized for their lack of interpretability and explainability.

% \kaleigh{TODO}: discussion of interpretability and explainability of deep nets

%They were first introduced in the deep neural network (DNN) literature by \cite{simonyan2013deep} and their use as explanations of network decisions has led to significant efforts in producing human-interpretable saliency maps. 
%In spite of their success with DNNs, the complexity rises in deep RL environments where decisions in aggregate correspond to agent behavior over temporally extended sequences of frames. %Some researchers have attempted to use saliency maps to provide evidence for explanations of agent behavior in deep RL \citep{greydanus2017visualizing, sundar2018transparency, iyer2018transparency}.

% This is different from image classification tasks where the network is typically provided a single image as input. Deep RL agents are structured differently to explore an environment, such as an Atari game, during training and expected to learn a policy. Thus, explanations in this context require more complex reasoning as they are derived from a temporal sequence of actions

%To generate interventional data, we use Toybox, a fully parameterized implementation of three Atari games \citep{foley2018toybox}. This provides a novel framework for evaluating saliency maps under intervention for RL environments. 
% We conducted a survey to better understand the ways in which saliency maps have been used as evidence in explanations of deep RL agents and found that saliency maps have been used to support explanations relating to semantic concepts of RL environments.
%Our survey suggests that saliency maps are often used for two main tasks: (1) assessing the RL agent's learned representations of semantic concepts, and (2) identifying the semantic features used for policy construction.

%Since saliency maps in deep RL are derived from a stack of temporally contiguous frames, 
% Since understanding environment semantics is particularly important for the success of deep RL agents, ascribing meaning to pixel-level interventions requires more scrutiny; 
%Our survey finds that saliency maps have been used to support explanations relating to semantic concepts of RL environments. However, the results communicated with saliency maps may not apply to human-understandable concepts. 
% The explanations that researchers frequently derive from saliency maps may not correspond to semantic concepts and features of RL environments. If saliency maps do not reflect the interventional relationships that are assumed by some researchers, incorrect, extrapolated conclusions may be drawn from the resulting maps.

% motivation
% \textbf{Survey of Usage of Saliency Maps.} We conducted a survey of how the deep RL community uses saliency maps and found that the explanations derived from saliency maps are often unfalsifiable, and can be highly subjective given the volume of conceptual information in image-based RL environments. We hypothesize that saliency maps are not self-sufficient to interpret RL agents and must be used with other evaluation methods.

%\textbf{Causal Explanations from Saliency Maps.}  %If saliency maps are used as tools of explanation, they should reflect causal relationships between the RL environment and the agent's behavior. 

% \textbf{Assessing Learned Representations from Saliency.} The explanations derived from saliency maps typically involve \textit{semantic}, human-understandable concepts. That is, salient pixels are typically mapped directly to semantic concepts in a game. However, the literature offers limited evidence that saliency maps are causally dependent on representations of human-understandable concepts. Recent work provides evidence for deep networks and humans having different visual inspectors \citep{}.

% \textbf{Assessing Inferred Policy Construction from Saliency.}


%approach
% \textbf{Example.} Consider the causal graphical model in Figure \ref{simple_gm} for an Atari game. The RL framework consists of the environment (in blue) and system (in yellow). In the environment, the \textit{pixel input} is generated from the underlying \textit{game state}. Then, pixel input and the \textit{learned network} are used to predict \textit{logits}, the raw probabilities over the output space. \textit{Saliency maps} are generated from the output of these logits and logits in aggregate also influence the agent's \textit{behavior}, such as "aiming". The game state affects \textit{semantic concepts} of the game. Together, saliency maps, behavior and semantic concepts are typically employed to generate explanations or \textit{claims} about agent behavior over temporally extended sequences.

% As described above, researchers assume saliency maps have a causal relationship with an agent's behavior and its environment. However, to the best of our knowledge, there is little evidence supporting this assumption. To test this hypothesis, we intervene on the common cause of behavior and saliency maps by following the causal chain back to game state. We intervene on game state, which is typically latent, using Toybox such that the underlying behavior holds true for a temporally extended sequence of frames. If the saliency maps do reflect this change, we can reject our hypothesis. Similarly, we can also verify how well semantic concepts correlate with salient pixels.

% Our experiments show some interesting results. TODO: add summary of results.

% outline, can be optional depending on venue/audience 
% Our paper proceeds as follows: ...

%It is noteworthy that all three of these components are connected only via common causes (i.e. pixel input and model). Hence, a connection between the components does not imply that a causal relationship exists. This alludes to the importance of assessing the degree to which saliency maps meet the assumptions outlined in section \ref{sec-inadeq} to determine whether saliency maps are good explanatory tools.


\subsection{Saliency Maps}
%Background on SMs
\subsubsection{Saliency Maps in Computer Vision}
% Saliency maps in the supervised DNN literature can be categorized into two categories.

\textbf{Gradient-Based Saliency.} Saliency maps were introduced by \citet{simonyan2013deep} to determine what pixels of an image are the most relevant to the network's decision. This involves calculating the gradient of the output with respect to the input.
%Using un-normalized scores of all the classes $S_c$ from a forward pass of the DNN, the authors back-propagate on the gradients with respect to the input $I$, $w_{ij}^c = \frac{\partial S_c}{\partial I} \arrowvert_{I_0}$, to get the pixel saliency at location $(i,j)$. A class saliency map can be generated by normalizing over the image for all pixel locations: $M_c(i,j) = \frac{w_{ij}}{\sum_{ij} w_{ij}}$. 
Following \cite{simonyan2013deep}, a multitude of gradient-based methods have been developed for DNNs with the intention of getting more realistic and understandable saliency maps \citep{simonyan2013deep, springenberg2014striving, shrikumar2017learning, smilkov2017smoothgrad, selvaraju2017grad, zhang2018top}. %For instance, Guided Backpropagation \citep{springenberg2014striving}, DeepLIFT \citep{shrikumar2017learning}, SmoothGrad \citep{smilkov2017smoothgrad}, Grad-CAM \citep{selvaraju2017grad} and most recently, Excitation Backpropagation \citep{zhang2018top} have been introduced.

\textbf{Perturbation-Based Saliency.} An alternative to gradient-based saliency map methods is perturbation-based methods. They were developed to measure how a change in conceptual parts of the input alters the network's output \citep{zeiler2014visualizing}. However, a common issue with this approach is it is difficult to perturb an area without introducing new information. Various other methods have been introduced to perturb pixels such that minimal new information is introduced \citep{ribeiro2016should, dabkowski2017real, fong2017interpretable}.  %This was first introduced by \cite{zeiler2014visualizing}, where the authors introduced masking portions of an image with gray squares to identify whether the network is using objects or the surrounding context. However, a common issue is this introduces new information, which hinders with the reasoning behind perturbing. Another variant of this is perturbation-based pixel saliency \citep{ribeiro2016should}. Advanced masking methods have been introduced by \cite{dabkowski2017real}, and \cite{fong2017interpretable}. Both of these use masked interpolation through an image to introduce minimal new information with the perturbation.

Background

% \section{Background}
% %Background on deep RL
% \subsection{Deep Reinforcement Learning}
% Reinforcement learning is a subfield of machine learning interested in training an agent to act in an environment through interaction. Certain states in the environment give the agent positive or negative reward. The agent learns a \emph{policy}, a mapping between states $S$ and actions $A$ according to reward signals $r \in R$. The goal is to learn a policy $\pi$ that maximizes the discounted sum of rewards received while acting in the environment \citep{sutton1998reinforcement}. 

% Deep reinforcement learning uses deep neural networks to represent policies. These models enable interactions using high-dimensional state inputs (e.g., images). % the hope is that it learns its own visual features for policy representation


%Use of SMs in the RL community.
% \subsection{Saliency Maps in Deep RL} 
% There is a growing use of saliency maps in deep RL. We consider four general categories of saliency maps in deep RL.
%There are a few saliency map methods available in this paradigm.

% \textbf{Jacobian Saliency.} Jacobian saliency maps, an application of regular gradient-based saliency maps, have been used to visualize the outputs of DQNs and generate explanations \citep{wang2015dueling, zahavy2016graying, bogdanovic2015deep}. However, as \cite{sundar2018transparency} point out, gradient-based methods in DNNs approximate linear decision boundaries and this does not produce interpretable saliency maps in deep RL because the mapping from states to actions is highly diverse unlike input image to class label mapping in classification tasks.
% %Sundar et al: "Pixel saliency makes linear approximations of the decision boundary and hence com-putes only local gradients.   GradCAM combines class specific gradient informationflowing into the last convolutional layer of the CNN. While this is useful for super-vised learning, this may not yield good saliency maps for reinforcement learning. Thisis because the reinforcement learning networks are not trained for an input image toclass label mapping and there is a high diversity in the input states for which the net-work chooses an action label “UP” for instance. "
% % \citet{sundar2018transparency} showed multiple gradient-based saliency maps on Atari testbeds and their substantially differing resulting interpretations. 
% Thus, merely porting saliency map methods from supervised contexts to deep RL does not fulfill the purposes that explanations in RL require. In this work, we use Jacobian saliency maps as the baseline. 

% \textbf{Perturbation Saliency.} Recognizing the lack of interpretability in Jacobian saliency methods, \citet{greydanus2017visualizing} developed a perturbation-based method to generate saliency videos of deep RL agents. They perturb the original input image using a Gaussian blur of the image generated by the Hadamard product and measure changes in policy from removing information from a region. TODO: add details how this is a less fat-handy perturbation and why that is important in the case of RL.

% \textbf{Object Saliency.} Noting the importance of objects in RL testbeds, \citet{iyer2018transparency} developed an object-sensitive saliency visualization method. They use template matching, a common computer vision technique, to detect (template) objects within an input image and store these in \textit{object channels} in the input image alongside the RBG channels. To generate object sensitive saliency maps, they mask each object with the background image and compute the difference in Q-values of the unmasked and masked states. The difference in Q-values represent the influence of the object on the Q-value.

% \textbf{Attention Saliency.} Most recently, attention-based methods have been proposed to generate interpretable saliency maps \citep{mott2019towards, nikulin2019free}.

% Saliency map methods typically use backpropogation of activations to identify parts of the images most important to making the agent’s decision. Briefly describe:
% \begin{itemize}
%     \item Jacobian methods
%     \item perturbation methods
%     \item the type surviving the Kim et al 2018 analysis (Guided Backprop?) \citep{adebayo2018sanity}
% \end{itemize}

% Saliency maps have been used to support explanations of agent behavior in RL applications \citep{}. Discussion:
% \begin{itemize}
%     \item why the temporal component makes reasoning harder in general; especially so in the case of porting SM methods from supervised contexts to RL
%     \item what methods are used/available in this paradigm 
%     \item use in the RL community for explanation 
% \end{itemize}

\subsection{Evaluation of Semantic Concepts in Saliency Maps}
To identify when there is a relationship between semantic concepts and saliency, we empirically evaluate the counterfactual importance of each semantic concept. We first identify semantic concepts using the extended graphical models (see appendix). We then design and run 50 samples of each intervention for each semantic concept. The interventions are run with varying intensities for 150 timesteps. See Table \ref{interventions} for a description of the interventions.

\begin{table}
\centering
\begin{tabular}{ |c|c|c| } 
 \hline
     & \textbf{Concepts} & \textbf{Intervention} \\ 
 \hline
 \textbf{Breakout} & Ball & \textbf{(1)} move ball position between [5,15] pixels; \textbf{(2)} increase ball speed by [1,3]. \\ 
  & Paddle & \textbf{(1)} move paddle position between [5,15] pixels to left or right. \\ 
  & Bricks & \textbf{(1)} invert bricks; \textbf{(2)} remove 5 random bricks; \textbf{(3)} remove a random row. \\ 
 \hline
 \textbf{Amidar} & Player & 4  \\ 
  & Enemies & 36 \\
  & Tiles & 36 \\
 \hline
\end{tabular}
\caption{Interventions for identifying CFi for each semantic concept.}
\label{interventions}
\end{table}

The results for the relationship between CFi and saliency in Breakout are shown for each intervention in Figure \ref{breakout_cfi_corr}. TODO: explain results. 

Similar experiments are done for Amidar (see appendix X). We find...TODO: explain results for Amidar. 

It could be that the relationship between CFi and saliency only holds at certain time periods (i.e. when ball is near the paddle in Breakout). To identify this, we assess if there is a pattern between CFi and salient over time. The results can be found in Figure \ref{}. We expect to see that CFi and saliency peak at the same time for the causal relationship to hold. TODO: explain results.

\begin{figure}
    \hspace*{-1cm}        
    \centering
    \includegraphics[width=\linewidth]{figures/breakout_CFi_saliency_corr_50s.png}
    \caption{Counterfactual importance vs saliency for (a) perturbation saliency; (b) object saliency; (c) Jacobian saliency.}
    \label{breakout_cfi_corr}
\end{figure}


%Reinforcement learning is complicated, and deep networks are complicated. There is a real need for explanation in these systems. Deep models in reinforcement learning are used for selecting actions over temporally extended periods. The temporal and interactive nature of RL systems present a different set of opportunities and challenges in explanations of behavior. Given the development and use of saliency maps to support explanations of agent behavior in deep RL applications, the use of saliency maps as tools of explanation in RL deserves its own evaluation.

\begin{figure}
\centering
	\begin{minipage}{.3\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/breakout_control.png}
		%\caption{original}
		\label{fig:breakout_control}
		\end{minipage}
%
	\begin{minipage}{.3\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/breakout_reflect.png}
		%\caption{reflected}
		\label{fig:breakout_reflect}
	\end{minipage}
	
	\begin{minipage}{.3\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/breakout_reflect_bp.png}
		%\caption{reflected}
		\label{fig:breakout_reflect_bp}
	\end{minipage}
\caption{(a) A perturbation saliency map from a frame in Breakout, and (b) a saliency map from the same model on the same frame with the brick patterned reflected across the vertical axis. \akanksha{The red regions indicate areas of the image that represent rewards, and blue regions indicate areas of the image that represent actions}. The pattern and intensity of saliency around the channel is not symmetric. In Section \ref{sec:case-study-1}, we examine whether reflecting the ball and paddle positions with the brick configuration increases the saliency of the reflected channel. }
\label{fig:breakout_example}
\end{figure}

\section{Generating Claims}
Note the inverse of the proposed approach is \textit{sufficiently causal}: TODO: give definition. If the agent has learned representation $R$, the pixels corresponding to the learned representation will always be salient. However, another learned representation may result in saliency on the same set of pixels. Researchers are instead interested in inferring what the agent has learned using saliency. This is also known as inferring \textit{causes of effects}. 

\textbf{Assessing Policy Construction.}
% The survey reveals that researchers associate intent behind policy construction and associate behavioral features. 
The policy a deep RL agent learns during training is guided by reward signals in the environment. These reward signals map to how the semantic features in the game evolve. By definition, these representations are causal for the network's output and are consequently reflected in saliency maps. However, given the many-to-many mapping between semantic concepts...
% The policy a deep RL agent learns during training contains what humans see as behavioral features. These representations are causal for the network's output and are consequently reflected in saliency maps. However, there are various other associational representations that can be speculated from a saliency map despite them not existing in the learned policy. \cite{???} provided evidence that humans are more susceptible to identifying spurious correlations. This suggests that any human reasoning requires complex interpretation to assess learned representations from saliency maps.

\textbf{Assessing Learned Representations.}
Prior studies have provided evidence that humans rely on references to semantic, human-understandable concepts. \cite{tenenbaum2003learning} demonstrate that humans organize objects based on their causal properties and inherently form abstract categories. \cite{dubey2018investigating} further show that humans use semantic concepts to develop a strategy to play games. Similarly, the survey reveals that humans look at saliency maps and interpret a strategy by associating salient pixels with concepts they know of. However, there is little evidence that saliency maps are capable of representing complex semantic-level representation.

\section{Assumptions}
To interpret saliency maps as explanatory tools for deep RL, researchers typically make the following assumptions. 
First, saliency maps indicate constraints on the space of possible policies. For instance, the example above uses saliency to assess that the agent has learned to ``target bricks with higher reward.''
Second, salient regions capture representations of semantic concepts learned by the network. 
For instance, the salient region above the tunnel being created in Figure \ref{fig:breakout_example}a can easily be interpreted to indicate the importance of tunnels to the agent.

\section{CF Importance}
%CF importance; what matters and what doesn’t for agent
% \textbf{Evaluating Existence of Semantic Concepts in Saliency Maps.} To evaluate the relationship between semantic concepts and saliency maps, we propose identifying the \textit{counterfactual importance} of each semantic concept. We define counterfactual importance (CFi) as $CFi (A_f, A_c) = \sqrt{\sum_{i=0}^{n} (A_f(i) - A_c(i))^2}$ where $A_f$ and $A_c$ are the probability distributions over the set of actions for a factual and counterfactual state respectively, and $n$ is the number of actions. Counterfactual importance intuitively reflects what is significant to the agent versus what is not at a given state. We expect that if a semantic concept is highly salient, intervening on it should result in a different distribution over actions (i.e. CFi). If the intervention causes a higher CFi for a highly salient ojbect, this implies that there is a causal relationship the semantic concept and saliency. We can similarly calculate the counterfactual importance using the value output.

% Figures \ref{amidar_score_ex_pert} and \ref{amidar_score_ex_jac} show the result of intervening on displayed score on reward and saliency intensity for the first 1000 timesteps of an episode. The mean is calculated over 50 samples. If an agent died before 1000 timesteps, the last reward was extended for the remainder of the timesteps and saliency was treated to be non-existent (ie. 0).  %show a contradicting example of saliency maps not being causally affected by agent behavior. That is 

% Using rewards as a proxy for agent behavior, we can conclude that different interventions on score produce contrasting agent behavior. This is evident from rewards differing over time for all the interventions due to early agent death.
% However, salience intensity patterns of all interventions follow very closely to the original trajectory. Since various interventions on displayed score cause degraded performance (Figure \ref{amidar_score_ex_obj}b) despite resulting in similar saliency maps (Figure \ref{amidar_score_ex_obj}c), we can conclude that we cannot assess the agent's behavior using just saliency intensity.
